List-Decodable Covariance Estimation

We give the first polynomial time algorithm for \emph{list-decodable covariance estimation}. For any $\alpha > 0$, our algorithm takes input a sample $Y \subseteq \mathbb{R}^d$ of size $n\geq d^{\mathsf{poly}(1/\alpha)}$ obtained by adversarially corrupting an $(1-\alpha)n$ points in an i.i.d. sample $X$ of size $n$ from the Gaussian distribution with unknown mean $\mu_*$ and covariance $\Sigma_*$. In $n^{\mathsf{poly}(1/\alpha)}$ time, it outputs a constant-size list of $k = k(\alpha)= (1/\alpha)^{\mathsf{poly}(1/\alpha)}$ candidate parameters that, with high probability, contains a $(\hat{\mu},\hat{\Sigma})$ such that the total variation distance $TV(\mathcal{N}(\mu_*,\Sigma_*),\mathcal{N}(\hat{\mu},\hat{\Sigma}))<1-O_{\alpha}(1)$. This is the statistically strongest notion of distance and implies multiplicative spectral and relative Frobenius distance approximation for parameters with dimension independent error. Our algorithm works more generally for $(1-\alpha)$-corruptions of any distribution $D$ that possesses low-degree sum-of-squares certificates of two natural analytic properties: 1) anti-concentration of one-dimensional marginals and 2) hypercontractivity of degree 2 polynomials. Prior to our work, the only known results for estimating covariance in the list-decodable setting were for the special cases of list-decodable linear regression and subspace recovery due to Karmarkar, Klivans, and Kothari (2019), Raghavendra and Yau (2019 and 2020) and Bakshi and Kothari (2020). These results need superpolynomial time for obtaining any subconstant error in the underlying dimension. Our result implies the first polynomial-time \emph{exact} algorithm for list-decodable linear regression and subspace recovery that allows, in particular, to obtain $2^{-\mathsf{poly}(d)}$ error in polynomial-time. Our result also implies an improved algorithm for clustering non-spherical mixtures.

==> content/final-algo.tex <==
%!TEX root = ../main.tex
\section{List-Decodable Covariance Estimation} 
Our algorithm takes input an $(1-\alpha)$-corruption of an i.i.d. sample $X$ of $\poly_{\alpha}(d)$ size and succeeds whenever the original uncorrupted sample satisfies some natural deterministic conditions inherited from the underlying distribution $D$. We call such samples ``good''. % required in the input (uncorrupted) sample under which our algorithm succeeds. 

 \begin{definition}["Good" Sample]
  \label{defn:good-sample}
      Let $D$ be a zero-mean probability distribution on $\R^d$ with a positive definite covariance.
      Suppose further that for some $C>0$, $D$ is $s(\delta)$-certifiably $(C/2,\delta)$-anti-concentrated for $s(\delta) = C/\delta^2$ and has certifiably $C/2$-hypercontractive degree $2$ polynomials. We will abbreviate $s(\delta)$ to $s$ below:

      A collection of points $X = \{x_1, x_2, \ldots, x_n\} \subseteq \bbQ^d$ of size $n$ with empirical covariance $\Sigma_*$ is said to be a \emph{good sample for $D$} if $\Sigma_*= \frac{1}{n} \sum_i x_i x_i^{\top}$ satisfies:
      \begin{enumerate}
        %\item Empirical mean: $\Iprod{\hat{\mu},v}^2 \leq 0.1 v^{\top} \Sigma_\ast v$ % \sqrt{\frac{\trace{\Sigma_{\ell}} }{m_\ell n}} + \sqrt{\frac{\|\Sigma_{\ell}\|_2d}{m_{\ell n}}}$
        \item Spectral Convergence: $ 0.5 \E_D xx^{\top} \preceq \Sigma_* \preceq 1.5 \E_D xx^{\top}$.

        \item Frobenius Convergence: $\Norm{\Sigma_*^{-1/2} \Paren{\frac{1}{n} \sum_i x_i x_i ^{\top}} \Sigma_*^{\dagger/2} - I}_F \leq 1$.

        \item Certifiable Anti-concentration: For $\delta = \alpha^{10}$ \FIXME{check},
        % \begin{enumerate}
        %   \item For all $x_i \in C_{\ell}$, \[ \forall v\in \mathbb{R}^d,
        %     \norm{v}_2^{2t-2} \Iprod{x_i,v}^2 +\gamma_3^2 p^2 (\Iprod{\Sigma_{\ell}^{-\frac{1}{2}} x_i,v})
        %     \geq \gamma_3^2 \norm{v}_2^{2t}
      %     \]
      \[
      \sststile{2s}{v} \Set{
      \frac{1}{n}\sum_{\substack{ i \leq n} } q^2_{\delta, \Sigma_*} \Paren{x_i,v } \leq C \delta \Paren{v^{\top}\Sigma_* v}^{s}}\mper
      \]
      
      % \[
      % \sststile{2s}{v} \Set{
      % \frac{k}{n}\sum_{\substack{ i_1, i_2 \in C_r, j_1, j_2 \in C_{r'}}}  q^2_{\tau, \hat{\Sigma}(r)} \Paren{x_{i_1} -x_{i_2} -x_{j_1} + x_{j_2},v } \leq 10C\tau \Paren{v^{\top}(\hat{\Sigma}(r) + \hat{\Sigma}(r') v}^{2s}_2}
      % \]
      
      \item Certifiable Hypercontractivity: For every $j \leq s$, \FIXME{check, may not need $j \leq s$.}
      \[
      \sststile{2s}{Q} \Set{
      \frac{1}{n} \sum_{\substack{ i\leq n}}  \paren{x_i^{\top}Qx_i-\frac{1}{n} \sum_{i \leq n} x_i^{\top}Qx_i}^{2j}
           \leq (Cj)^{2j} \Norm{\Sigma_*^{\frac{1}{2}}Q\Sigma_*^{\frac{1}{2}}}_F^{2j}}\mper
      \]
      \end{enumerate}
\end{definition}

\begin{lemma}[Rational Truncations of Random Samples are Good] \label{lem:typical-samples-are-good}
Let $D$ be a $0$ mean distribution on $\R^d$ that is $s(\delta)$-certifiably $(C/2,\delta)$-anti-concentrated and certifiably $(C/2)$-hypercontractive. Suppose $I\succeq \E_D xx^{\top} \succeq 2^{-d^B}I$. Let $X_{untruncated} = \{x_1', x_2',\ldots, x_n'\}$ be an i.i.d. sample from $D$. Let $X= \{x_1,x_2,\ldots, x_n\}$ be obtained by truncating each $x_i$ to a rational number such that $\norm{x_i - x_i'}_2\leq 2^{-d^{2B}}$ for every $1 \leq i \leq n$. Then, with probability at least $1-1/d^{100}$ over the draw of $X_{untruncated}$, for all $n \geq d^{??}$, $X$ is a good sample for $D$. 
\end{lemma}

\begin{remark}
Observe that the definition of a good sample asks for a subset of points with rational coordinates. This is essentially\footnote{In principle, one could have sophisticated finite bit-length representations for irrational numbers that lie in, say, some chosen extension field of rationals.} necessary (and almost always, implicit) in algorithms that are implementable in the standard Turing Machine model. For reasons discussed in Section~\ref{}, we choose to be explicit about such numerical issues in this work. An i.i.d. sample from distribution $D$ will, in general, have points with irrational coordinates and thus \emph{does not} satisfy our definition of a good sample. One might reasonably imagine that replacing each point in an i.i.d. sample by some reasonable rational approximation should be enough to obtain a good sample. While this provably fails without further assumptions, it is indeed true if we assume an inverse exponential $2^{-d^{2B}}$ lower bound on the smallest eigenvalue of $\E_D xx^{\top}$, then the truncated rational $x_i$s need at most $d^{O(B)}$ bits to describe (see proof of Lemma~\ref{lem:typical-samples-are-good}). Notice that this eigenvalue lower bound is an extremely mild assumption (in contrast to, say, a $\poly(d)$ upper-bound on the condition number, we only assume an exponential upper-bound on the condition number). We show later that we do not need such a lower-bound without hurting the performance of our algorithm whenever $D$'s covariance can be sandwiched (in Löwner ordering) by small multiples of some positive semidefinite matrix with \emph{rational} entries. Such an assumption is necessary to handle, for e.g., rank deficient covariances and without it, it is provably impossible for any algorithm (however inefficient) to provide guarantees in total variation distance as in our work. We stress that the numerical issues discussed here are unrelated to the issue of approximately solving SDPs and are entirely because rational truncations of input points can alter the kernel of the unknown covariance while exactly recovering the kernel exactly is necessary for recovering covariances that are close to the truth in Löwner order.
\end{remark} 

